Perturbed, Entropy-Based Closure for Radiative Transfer

We derive a hierarchy of closures based on perturbations of well-known entropy-based closures; we therefore refer to them as perturbed entropy-based models. Our derivation reveals final equations containing an additional convective and diffusive term which are added to the flux term of the standard closure. We present numerical simulations for the simplest member of the hierarchy, the perturbed M1 or PM1 model, in one spatial dimension. Simulations are performed using a Runge-Kutta discontinuous Galerkin method with special limiters that guarantee the realizability of the moment variables and the positivity of the material temperature. Improvements to the standard M1 model are observed in cases where unphysical shocks develop in the M1 model.

==> sections/acknowledgement.tex <==
\section*{Acknowledgement}
%
The authors would like to thank Dave Levermore, who motivated
this work, and Ryan G. McClarren for providing the $P_{99}$ transport solution
which was used for comparisons in Section~\ref{sec_results_sub:marshak}.  The
author's would also like to express their appreciation for the
hospitality provided by the Institute for Pure and Applied Mathematics (IPAM),
where this work was originated.


